Phoneme Boundary Detection using Learnable Segmental Features

Phoneme boundary detection plays an essential first step for a variety of speech processing applications such as speaker diarization, speech science, keyword spotting, etc. In this work, we propose a neural architecture coupled with a parameterized structured loss function to learn segmental representations for the task of phoneme boundary detection. First, we evaluated our model when the spoken phonemes were not given as input. Results on the TIMIT and Buckeye corpora suggest that the proposed model is superior to the baseline models and reaches state-of-the-art performance in terms of F1 and R-value. We further explore the use of phonetic transcription as additional supervision and show this yields minor improvements in performance but substantially better convergence rates. We additionally evaluate the model on a Hebrew corpus and demonstrate such phonetic supervision can be beneficial in a multi-lingual setting.

==> 5_analysis.tex <==
\vspace{-0.3cm}
\section{Cross-language phoneme boundary detection}
\vspace{-0.3cm}

%\subsection{Hebrew corpus experiments}

One concern when using the phoneme classification loss is convergence to a language-dependent model. To further explore that we evaluated the performance of two models that were trained on American English (TIMIT) and tested on a Hebrew language corpus~\cite{benautomatic}. The Hebrew language has only partial overlap in its phonetic set to English, and the utterances in the Hebrew corpus consist of both read and spontaneous speech. Results are summarized in Table \ref{tab:heb}.

\noindent Interestingly, results suggest that incorporating the phoneme classification loss with segmental features slightly improved overall performance in comparison to using segmental features alone. An example of the model predictions together with the target label is depicted in Figure~\ref{fig:spect}.

\begin{table}[t]
\vspace{-0.4cm}
    \small
	\centering
	\caption{An ablation study on the effect of the \phn loss on Hebrew language.}
  \vspace{5pt}
  \label{tab:heb}
  \begin{tabular}{l|ccccc}
    \toprule
	Model & P & R & F1 & R-val  \\
    \midrule
       \segfeat w/o~  \phn Loss   & \textbf{83.58} & 79.2 & 81.24 & 83.67 \\
       \segfeat w~ \phn Loss   & 83.11 & \textbf{81.66} & \textbf{82.38} & \textbf{84.92} \\
    \bottomrule
  \end{tabular}
  \vspace{-0.1cm}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{images/spect_viz_1.pdf}
\vspace{-0.9cm}
\caption{Example of segmentation result on an Hebrew utterance using an English trained model.}
\label{fig:spect}
\end{figure}


==> __latexindent_temp.tex <==
     0ms  & 74.0 & 70.0 & 73.0 & 76.0   \\
    & 10ms  & - & 79.1 & 78.16 & 81.11   \\
    & 20ms  & 74.8 & 81.9 & 78.2 & 80.1  \

==> introduction.tex <==
\section{Introduction}

% General statement
\IEEEPARstart{S}{peech} segmentation is a crucial step in many speech recognition and speech analysis tasks; that is, breaking a speech utterance into contiguous, arbitrary-length segments.

% Applications of speech segmentation
There are several segmentation tasks in the speech domain.
In phoneme segmentation, a contiguous speech utterance is broken down into phone units \cite{keshet2005phoneme, king2013accurate, hoang2015blind, michel2017blind}, which is an essential first step for many automatic speech recognition (ASR) tasks. Other segmentation models can be used for cleaning speech data by removing non-speech regions such as noise or music \cite{kubala1996transcribing, rybach2009audio}.
Another form of speech segmentation can be used to detect the boundaries of a phonetic property and can thereby measure its duration \cite{sonderegger2012automatic, adi2016prevoicing, adi2016vowel}. Automatically annotating and measuring phonetic properties of speech is an important task for many theoretical and clinical studies. It replaces the labor-intensive manual annotation process that is commonly carried out by researchers, and allows efficient processing of large amounts of data.

% Previous work (TODO extend)
Several previous attempts aimed to perform segmentation of speech using machine-learning techniques. These attempts usually involve classic algorithms such as hidden Markov models and Structured SVM, and are based on handcrafted feature functions that should be specifically and separately designed for each task  \cite{toledano2003automatic, keshet2007large, sonderegger2012automatic}. Other works use deep learning based methods for segmentation. However, rather than predicting the segmentation as a whole, they are usually based on a frame-based model that predicts class probabilities for each frame \cite{adi2016automatic, franke2016phoneme, michel2017blind}.

% Novel approach for speech segmentation
We tackle this problem by designing a Recurrent Neural Network (RNN)-based feature function that is trained jointly with the structured objective. More specifically, our novel network architecture encodes a proposed segmentation by traversing its segments in several different ways \comment{what do this mean?}, forming a powerful feature representation that is then scored using a feedforward neural network. Since the amount of possible segmentation is exponential, we use a dynamic programming algorithm that exploits the dependencies within the data, and performs inference in practical time, both when the number of segments are known and when they vary.

% Results (TODO)

\comment{TODO: finish.}

% Goal definition

% What is planned


 
